Recognition of Logically Related Regions Based Heap Abstraction

This paper presents a novel set of algorithms for heap abstraction, identifying logically related regions of the heap. The targeted regions include objects that are part of the same component structure (recursive data structure). The result of the technique outlined in this paper has the form of a compact normal form (an abstract model) that boosts the efficiency of the static analysis via speeding its convergence. The result of heap abstraction, together with some properties of data structures, can be used to enable program optimizations like static deallocation, pool allocation, region-based garbage collection, and object co-location. More precisely, this paper proposes algorithms for abstracting heap components with the layout of a singly linked list, a binary tree, a cycle, and a directed acyclic graph. The termination and correctness of these algorithms are studied in the paper. Towards presenting the algorithms the paper also presents concrete and abstract models for heap representations.

==> DAG.tex <==
\begin{center}
\begin{picture}(112,20)(0,0)
\put(-10,10){\circle{5}}
\put(-9,11){\makebox[0pt]{\raisebox{-1ex}{{\small s }}}}
\put(-7.5,10.5){\vector(1,0){6}} \put(32,20){\oval(7,5)}
\put(29,18){\vector(-4,-1){24}}\put(29,18){\vector(-2,-1){12}}
\put(29,18){\vector(-1,-2){2.7}}\put(33,17.5){\vector(1,-2){2.7}}
\put(33,17.5){\vector(2,-1){13.5}}\put(35,18){\vector(4,-1){24}}
\put(2,10){\oval(7,5)} \put(14,10){\oval(7,5)}
\put(26,10){\oval(7,5)} \put(38,10){\oval(7,5)}
\put(50,10){\oval(7,5)} \put(62,10){\oval(7,5)}
\put(29,2){\vector(-4,1){24}}\put(29,2){\vector(-2,1){12}}
\put(29,2){\vector(-1,2){2.7}}\put(33,2.5){\vector(1,2){2.7}}
\put(33,2.5){\vector(2,1){13.5}}\put(35,2){\vector(4,1){24}}
\put(32,0){\oval(7,5)}
\put(33,21){\makebox[0pt]{\raisebox{-1ex}{{\small $h_0$ }}}}
\put(3,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_1$ }}}}
\put(15,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_2$ }}}}
\put(27,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_3$ }}}}
\put(39,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_4$ }}}}
\put(51,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_5$ }}}}
\put(63,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_6$ }}}}
\put(33,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_7$ }}}}
%----------------------------------------------------------------
\put(80,10){\circle{5}}
\put(81,11){\makebox[0pt]{\raisebox{-1ex}{{\small s }}}}
\put(82.5,10.5){\vector(1,0){7}}\put(102,20){\oval(7,5)}
\put(99,18){\vector(-1,-2){3}}\put(104,17.5){\vector(1,-1){5}}
\put(93,10){\oval(7,5)}
\put(111,10){\oval(12,5)}\put(110,12.5){{\large $\curvearrowright$}}
\put(99,2){\vector(-1,2){3}}\put(104,2.5){\vector(1,2){2.5}}
\put(102,0){\oval(7,5)}
\put(103,21){\makebox[0pt]{\raisebox{-1ex}{{\small $i_0$ }}}}
\put(94,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_1$ }}}}
\put(112,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_2$ }}}}
\put(103,1){\makebox[0pt]{\raisebox{-1ex}{{\small $i_3$ }}}}
\end{picture}
\end{center}


==> bt.tex <==
\begin{center}
\begin{picture}(112,30)(0,0)
\put(-10,0){\oval(7,5)}\put(2,0){\oval(7,5)}\put(14,0){\oval(7,5)}
\put(26,0){\oval(7,5)}\put(38,0){\oval(7,5)}\put(50,0){\oval(7,5)}
\put(62,0){\oval(7,5)}\put(74,0){\oval(7,5)}
\put(-9,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_7$ }}}}
\put(3,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_8$ }}}}
\put(15,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_9$ }}}}
\put(27,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_{10}$ }}}}
\put(39,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_{11}$ }}}}
\put(51,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_{12}$ }}}}
\put(63,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_{13}$ }}}}
\put(75,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_{14}$ }}}}
%---------------------------------------------
\put(-3,10){\oval(7,5)}\put(20,10){\oval(7,5)}\put(44,10){\oval(7,5)}
\put(68,10){\oval(7,5)}\put(47.5,10){\vector(1,0){17}}
\put(-3,7.5){\vector(-1,-1){5}}\put(-3,7.5){\vector(1,-1){5}}
\put(20,7.5){\vector(-1,-1){5}}\put(20,7.5){\vector(1,-1){5}}
\put(44,7.5){\vector(-1,-1){5}} \put(44,7.5){\vector(1,-1){5}}
\put(68,7.5){\vector(-1,-1){5}} \put(68,7.5){\vector(1,-1){5}}
\put(-2,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_3$ }}}}
\put(21,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_4$ }}}}
\put(45,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_5$ }}}}
\put(69,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_6$ }}}}
%---------------------------------------------
\put(8,20){\oval(7,5)}\put(55,20){\oval(7,5)}
\put(8,17.5){\vector(-2,-1){10}} \put(8,17.5){\vector(2,-1){10}}
\put(55,17.5){\vector(-2,-1){10}} \put(55,17.5){\vector(2,-1){10}}
\put(9,21){\makebox[0pt]{\raisebox{-1ex}{{\small $h_1$ }}}}
\put(56,21){\makebox[0pt]{\raisebox{-1ex}{{\small $h_2$ }}}}
%---------------------------------------------
\put(32,30){\oval(7,5)} \put(10,30){\circle{5}}
\put(11,31){\makebox[0pt]{\raisebox{-1ex}{{\small R }}}}
\put(12.5,30){\vector(1,0){16}} \put(32,27.5){\vector(-4,-1){21}}
\put(32,27.5){\vector(4,-1){21}}
\put(33,31){\makebox[0pt]{\raisebox{-1ex}{{\small $h_0$ }}}}
%-------------------------------------------------------------------
%-------------------------------------------------------------------
\put(94,0){\oval(7,5)}\put(106,0){\oval(7,5)}\put(118,0){\oval(7,5)}
\put(130,0){\oval(7,5)}
\put(95,1){\makebox[0pt]{\raisebox{-1ex}{{\small $i_5$ }}}}
\put(107,1){\makebox[0pt]{\raisebox{-1ex}{{\small $i_6$ }}}}
\put(119,1){\makebox[0pt]{\raisebox{-1ex}{{\small $i_7$ }}}}
\put(131,1){\makebox[0pt]{\raisebox{-1ex}{{\small $i_8$ }}}}
%-------------------------------------------------------------------
\put(100,10){\oval(7,5)}\put(124,10){\oval(7,5)}\put(103.5,10){\vector(1,0){17}}
\put(100,7.5){\vector(-1,-1){5}}\put(100,7.5){\vector(1,-1){5}}
\put(124,7.5){\vector(-1,-1){5}}\put(124,7.5){\vector(1,-1){5}}
\put(101,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_3$ }}}}
\put(125,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_4$ }}}}
%-------------------------------------------------------------------
\put(90,20){\oval(15,5)}\put(112,20){\oval(7,5)}
\put(84,22.5){{\large $\curvearrowright$}} \put(90,22.5){{\large
$\curvearrowright$}}
\put(87,27){\makebox[0pt]{\raisebox{-1ex}{{\small l }}}}
\put(93,27){\makebox[0pt]{\raisebox{-1ex}{{\small r }}}}
\put(112,17.5){\vector(-2,-1){10}} \put(112,17.5){\vector(2,-1){10}}
\put(91,21){\makebox[0pt]{\raisebox{-1ex}{{\small $i_1$ }}}}
\put(113,21){\makebox[0pt]{\raisebox{-1ex}{{\small $i_2$ }}}}
%-------------------------------------------------------------------
\put(101,30){\oval(7,5)} \put(79,30){\circle{5}}
\put(80,31){\makebox[0pt]{\raisebox{-1ex}{{\small R }}}}
\put(81.5,30){\vector(1,0){16}} \put(101,27.5){\vector(-1,-1){5}}
\put(101,27.5){\vector(2,-1){10}}
\put(102,31){\makebox[0pt]{\raisebox{-1ex}{{\small $i_0$ }}}}
\end{picture}
\end{center}


==> cycle.tex <==
\begin{center}
\begin{picture}(62,22)(0,0)
\put(-10,20){\circle{5}} \put(-7.5,20){\vector(1,0){6}}
\put(2,10){\oval(7,5)}\put(26,10){\oval(7,5)}
\put(2,0){\oval(7,5)}\put(14,0){\oval(7,5)}\put(26,0){\oval(7,5)}
\put(-9,21){\makebox[0pt]{\raisebox{-1ex}{{\small s }}}}
\put(2,12.5){\vector(0,1){5}} \put(2,2.5){\vector(0,1){5}}
\put(2,20){\oval(7,5)}\put(5.5,20){\vector(1,0){5}}
\put(14,20){\oval(7,5)} \put(17.5,20){\vector(1,0){5}}
\put(26,20){\oval(7,5)}\put(26,17.5){\vector(0,-1){5}}
\put(26,7.5){\vector(0,-1){5}}\put(10.5,0){\vector(-1,0){5}}
\put(22.5,0){\vector(-1,0){5}} \put(5.5,10){\vector(1,1){7.5}}
\put(3,21){\makebox[0pt]{\raisebox{-1ex}{{\small $h_0$ }}}}
\put(15,21){\makebox[0pt]{\raisebox{-1ex}{{\small $h_1$ }}}}
\put(27,21){\makebox[0pt]{\raisebox{-1ex}{{\small $h_2$ }}}}
\put(3,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_7$ }}}}
\put(27,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_3$ }}}}
\put(3,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_6$ }}}}
\put(15,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_5$ }}}}
\put(27,1){\makebox[0pt]{\raisebox{-1ex}{{\small $h_4$ }}}}
%----------------------------------------------------------------
%----------------------------------------------------------------
\put(50,20){\circle{5}} \put(52.5,20){\vector(1,0){6}}
\put(51,21){\makebox[0pt]{\raisebox{-1ex}{{\small s }}}}
\put(62,20){\oval(7,5)}\put(65.5,20){\vector(1,0){5}}
\put(74,20){\oval(7,5)} \put(74,17.5){\vector(0,-1){5}}
\put(62,10){\oval(7,5)}\put(77,10){\oval(10,5)}
\put(76,12.5){{\large $\curvearrowright$}}
\put(62,12.5){\vector(0,1){5}}\put(65.5,10){\vector(1,1){7.5}}
\put(72,10){\vector(-1,0){6.5}}
\put(63,21){\makebox[0pt]{\raisebox{-1ex}{{\small $i_0$ }}}}
\put(75,21){\makebox[0pt]{\raisebox{-1ex}{{\small $i_1$ }}}}
\put(63,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_3$ }}}}
\put(78,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_2$ }}}}
\end{picture}
\end{center}


==> sll.tex <==
\begin{center}
\begin{picture}(112,10)(0,0)
\put(-10,10){\oval(7,5)} \put(-6.5,10){\vector(1,0){5}}
\put(-9,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_0$ }}}}
\put(-10,0){\circle{5}}
\put(-9,1){\makebox[0pt]{\raisebox{-1ex}{{\small s }}}}
\put(-10,2.5){\vector(0,1){5}}
\put(2,10){\oval(7,5)}\put(5.5,10){\vector(1,0){5}}
\put(3,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_1$ }}}}
\put(14,10){\oval(7,5)} \put(17.5,10){\vector(1,0){5}}
\put(15,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_2$ }}}}
\put(26,10){\oval(7,5)}\put(29.5,10){\vector(1,0){5}}
\put(27,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_3$ }}}}
\put(38,10){\oval(7,5)} \put(41.5,10){\vector(1,0){5}}
\put(39,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_4$ }}}}
\put(50,10){\oval(7,5)}\put(53.5,10){\vector(1,0){5}}
\put(51,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_5$ }}}}
\put(62,10){\oval(7,5)}
\put(63,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_6$ }}}}
\put(65.5,11){\vector(1,0){5}}\put(70.5,9){\vector(-1,0){5}}
\put(74,10){\oval(7,5)} \put(74,0){\circle{5}}
\put(75,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_7$ }}}}
\put(75,1){\makebox[0pt]{\raisebox{-1ex}{{\small e }}}}
\put(74,2.5){\vector(0,1){5}}
%----------------------------------------------------------------
\put(90,10){\oval(7,5)} \put(93.5,10){\vector(1,0){5}}
\put(91,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_0$ }}}}
\put(90,0){\circle{5}}
\put(91,1){\makebox[0pt]{\raisebox{-1ex}{{\small s }}}}
\put(90,2.5){\vector(0,1){5}} \put(102,10){\oval(7,5)}
\put(103,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_1$ }}}}
\put(100,12.5){{\large $\curvearrowright$}}
\put(105.5,10){\vector(1,0){5}} \put(114,10){\oval(7,5)}
\put(115,11){\makebox[0pt]{\raisebox{-1ex}{{\small $i_2$ }}}}
\put(117.5,11){\vector(1,0){5}}\put(122.5,9){\vector(-1,0){5}}
\put(126,10){\oval(7,5)} \put(126,0){\circle{5}}
\put(127,11){\makebox[0pt]{\raisebox{-1ex}{{\small $h_3$ }}}}
\put(126,1){\makebox[0pt]{\raisebox{-1ex}{{\small e }}}}
\put(126,2.5){\vector(0,1){5}}
\end{picture}
\end{center}

